LAB4D: A Low Power, Multi-GSa/s, Transient Digitizer with Sampling Timebase Trimming Capabilities

The LAB4D is a new application-specific integrated circuit (ASIC) of the Large Analog Bandwidth Recorder and Digitizer with Ordered Readout (LABRADOR) family, for use in direct wideband radio frequency digitization such as is used in ultrahigh energy neutrino and cosmic ray astrophysics. The LAB4D is a single channel switched-capacitor array (SCA) 12-bit sampler with integrated analog-to-digital converters (ADC), developed in the TSMC 0.25um process. The LAB4D, operating at 3.2GSa/s, contains 4096 total samples arranged in 32 windows, for a total record length of 1280ns. The 3dB bandwidth is approximately 1.3GHz, with a directly-coupled 50ohm input. This represents a factor of 16 increase in the sample depth and an increase in analog bandwidth and sampling depth in comparison to the previous generation LAB3 digitizer. Individually addressable windows allow for sampling and digitization to occur simultaneously, leading to nearly deadtime-free readout for kHz readout rates. All biases and current references are generated via internal digital-to-analog converters (DACs), resulting in a stand-alone digitizer with no additional support circuitry. In addition, the LAB4D contains sample cell timebase trimming capabilities, reducing the intrinsic sample-to-sample time variance to less than 5ps; an improvement of about 80%. This allows the LAB4D to be used in precision timing applications with minimal post-hoc calibration.

==> references.aux.tex <==
\begin{references}


@article{IceCube,
author={The IceCube Collaboration: M. G. Aartsen et al.},
  title={A Combined Maximum-likelihood Analysis of the High-energy Astrophysical Neutrino Flux Measured with IceCube},
  journal={The Astrophysical Journal},
  volume={809},
  number={1},
  pages={98},
  url={http://stacks.iop.org/0004-637X/809/i=1/a=98},
  year={2015}
}

@misc{gray_code,
  title={Pulse code communication},
  author={Gray, F.},
  url={https://www.google.com/patents/US2632058},
  year={1953},
  month=mar # "~17",
  publisher={Google Patents},
  note={US Patent 2,632,058}
}

@online{opencore,
  author = {Opencores},
  title = {OpenCores.org},
  year = 2015,
  url = {http://www.opencores.org},
  urldate = {2015-10-30}
}

@article{LAB3_design,
title = "The Large Analog Bandwidth Recorder and Digitizer with Ordered Readout (LABRADOR) ASIC",
author = "G.S. Varner and L.L. Ruckman and J.W. Nam and R.J. Nichol and J. Cao and P.W. Gorham and M. Wilcox",
journal = "Nucl. Instrum. Meth.",
volume = "A583",
pages = "447-460",
year = 2007
}

@inproceedings{RDC,
title = "A Study on the offset voltage of dynamic comparators",
author = "Ant\'{o}nio C. Pinto and Jorge R. Fernandes",
journal = "In Proceedings of Design of Integrated Circuits and Systems Conference (DCIS) 28th Ed.",
year = 2013
}

@article{RITC_design,
title = {A low-resolution, {GS}a/s streaming digitizer for a correlation-based trigger system},
author = {Kurtis Nishimura and Matthew Andrew and Zhe Cao and Michael Cooney and Peter Gorham and Luca Macchiarulo and Lisa Ritter and Gary Varner and Andres Romero-Wolf},
journal = {arxiv.org},
url = {http://arxiv.org/abs/1203.4178},
year = {2012}
}

@book{electronic_warfare,
title = {Electronic Warfare and Radar Systems Engineering Handbook},
author = {U.S. Navy},
publisher = {U.S. Navy's Weapons Division Avionics Department Electronic Warfare Division},
address = {Point Mugu, CA},
year = {1999}
}


@book{jackson,
title = {Classical Electrodynamics},
author = {Jackson, John David},
publisher = {John Wiley \& Sons, Inc.},
address = {New Jersey, USA},
edition = {3},
year = {1991}
}

@book{modern_astrophysics,
title = {An Interduction to Modern Astrophysics},
author = {B.W. Carroll \& D.A Ostlie},
publisher = {Pearson Education Inc.},
address = {San Francisco, CA, USA},
edition = {2},
year = {2007}
}

@article{PDG,
title = {Particle Data Group},
author = {J. Beringer et al.},
journal = {Phys. Rev. D},
volume = {86},
pages = {010001},
year = {2012}
}

@article{BZ_neutrino,
title = {Cosimc Rays at Ultra High energies (Neutrino?)},
author = {V.S. Berensinsky and G.T. Zatsepin},
journal = {Physics Letters},
volume = {28B},
pages = {423-424},
year = {1969}
}

@article{Swordy,
title = {The energy spectra and anisotropies of cosmic rays},
author = {S. Swordy},
journal = {Space Science Reviews},
volume = {99},
pages = {85-94},
year = {2001}
}

@misc{whanlon_swordy,
title = {Updated Cosmic Ray Spectra},
author = {W. Hanlon},
year = {2008},
url = {http://www.physics.utah.edu/~whanlon/spectrum.html},
note = {Accessed: 2015-01-22}
}

@article{Butterworth,
 title = {On the Theory of Filter Amplifiers},
  author = {S. Butterworth},
  journal = {Experimental Wireless \& the Wireless Engineer},
  volume = {7},
  pages = {536-541},
  year = {1930}
}

@article {Hess, 
	Author = {F. Hess, V.},
	Title = {About observations of the penetrating radiation in seven free Ballooning},
	Journal = {Physical magazine},
	Volume = {13},
	Pages = {1084--1091},
	Month = {November},
	Year = {1912}
} 
 
@misc{HessKol,
 	title = {Domenico Pacini, uncredited pioneer of the discovery of cosmic rays},
	author = {Alessandro De Angelis},
	journal = {Rivista del Nuovo Cimentro},
	volume = {33},
	pages = {713},
	year = {2010},
	url = {http://http://arxiv.org/abs/1103.4392}
}


@article{ANITAI_neutrino,
  title = {New Limits on the Ultrahigh Energy Cosmic Neutrino Flux from the ANITA Experiment},
  author = {Gorham, P. W. and Allison, P. and Barwick, S. W. and Beatty, J. J. and Besson, D. Z. and Binns, W. R. and Chen, C. and Chen, P. and Clem, J. M. and Connolly, A. and Dowkontt, P. F. and DuVernois, M. A. and Field, R. C. and Goldstein, D. and Goodhue, A. and Hast, C. and Hebert, C. L. and Hoover, S. and Israel, M. H. and Kowalski, J. and Learned, J. G. and Liewer, K. M. and Link, J. T. and Lusczek, E. and Matsuno, S. and Mercurio, B. C. and Miki, C. and Mio\ifmmode \check{c}\else \v{c}\fi{}inovi\ifmmode \acute{c}\else \'{c}\fi{}, P. and Nam, J. and Naudet, C. J. and Ng, J. and Nichol, R. J. and Palladino, K. and Reil, K. and Romero-Wolf, A. and Rosen, M. and Ruckman, L. and Saltzberg, D. and Seckel, D. and Varner, G. S. and Walz, D. and Wang, Y. and Wu, F.},
  collaboration = {ANITA Collaboration},
  journal = {Phys. Rev. Lett.},
  volume = {103},
  issue = {5},
  pages = {051103},
  numpages = {5},
  year = {2009},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.103.051103},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.103.051103}
}

@Article{Design:2008,
  author = 	 {ANITA Collaboration},
  title = 	 {The Antarctic Impulsive Transient Antenna Ultra-high Energy Neutrino Detector Design, Performance, and Sensitivity for 2006-2007 Balloon Flight},
  journal = 	 {Astroparticle Physics},
  year = 	 2009,
  volume =	 32,
  pages =	 {10-41}
}

@Article{Askaryan:2007,
  author = 	 {ANITA Collaboration},
  title = 	 {Observations of the {A}skaryan Effect in Ice},
  journal = 	 {Phys. Rev. Lett.},
  year = 	 2007,
  volume =	 99,
  pages =	 {171101}
}

@Article{CR:2010,
  author = 	 {Hoover S. et. al.},
  title = 	 {Observation of Ultra-high-energy Cosmic Rays with the ANITA Balloon-borne Radio Interferometer},
  journal = 	 {jas},
  year = 	 {1981},
  volume =	 {38},
  pages =	 {819-843}
}

@Article{askaryan_theory,
  author = 	 {G.A. Askar'yan},
  title = 	 {Excess Negative Charge of an Electron-Photon Shower and its Coherent Radio Emission},
  journal = 	 {JETP},
  year = 	 1962,
  volume =	 14,
  pages =	 {441-443}
}

@article{gzk_zatsepin,
      author         = "Zatsepin, G.T. and Kuzmin, V.A.",
      title          = "{Upper limit of the spectrum of cosmic rays}",
      journal        = "JETP Lett.",
      volume         = "4",
      pages          = "78-80",
      year           = "1966"
}

@article{gzk_greisen,
  title = {End to the Cosmic-Ray Spectrum?},
  author = {Greisen, Kenneth},
  journal = {Phys. Rev. Lett.},
  volume = {16},
  issue = {17},
  pages = {748--750},
  year = {1966},
  month = {Apr},
  doi = {10.1103/PhysRevLett.16.748},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.16.748},
  publisher = {American Physical Society}
}

@article{gorham_2010,
  title = {Observational constraints on the ultrahigh energy cosmic neutrino flux from the second flight of the ANITA experiment},
  author = {Gorham, P. W. and Allison, P. and Baughman, B. M. and Beatty, J. J. and Belov, K. and Besson, D. Z. and Bevan, S. and Binns, W. R. and Chen, C. and Chen, P. and Clem, J. M. and Connolly, A. and Detrixhe, M. and De Marco, D. and Dowkontt, P. F. and DuVernois, M. and Grashorn, E. W. and Hill, B. and Hoover, S. and Huang, M. and Israel, M. H. and Javaid, A. and Liewer, K. M. and Matsuno, S. and Mercurio, B. C. and Miki, C. and Mottram, M. and Nam, J. and Nichol, R. J. and Palladino, K. and Romero-Wolf, A. and Ruckman, L. and Saltzberg, D. and Seckel, D. and Varner, G. S. and Vieregg, A. G. and Wang, Y.},
  journal = {Phys. Rev. D},
  volume = {82},
  issue = {2},
  pages = {022004},
  numpages = {7},
  year = {2010},
  month = {Jul},
  doi = {10.1103/PhysRevD.82.022004},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.82.022004},
  publisher = {American Physical Society}
}

@article{gorham_2010_err,
  title = {Erratum: Observational constraints on the ultrahigh energy cosmic neutrino flux from the second flight of the ANITA experiment },
  author = {Gorham, P. W. and Allison, P. and Baughman, B. M. and Beatty, J. J. and Belov, K. and Besson, D. Z. and Bevan, S. and Binns, W. R. and Chen, C. and Chen, P. and Clem, J. M. and Connolly, A. and Detrixhe, M. and De Marco, D. and Dowkontt, P. F. and DuVernois, M. and Grashorn, E. W. and Hill, B. and Hoover, S. and Huang, M. and Israel, M. H. and Javaid, A. and Liewer, K. M. and Matsuno, S. and Mercurio, B. C. and Miki, C. and Mottram, M. and Nam, J. and Nichol, R. J. and Palladino, K. and Romero-Wolf, A. and Ruckman, L. and Saltzberg, D. and Seckel, D. and Shang, R. Y. and Varner, G. S. and Vieregg, A. G. and Wang, Y.},
  journal = {Phys. Rev. D},
  volume = {85},
  issue = {4},
  pages = {049901},
  numpages = {2},
  year = {2012},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.85.049901},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.85.049901}
}

@article{Varner_2003,
  title = {Monolithic Multi-channel GSa/s Transient Waveform Recorder for Measuring Radio Emissions from High Energy Particle Cascades},
  author = {Gary S. Varner, Peter Gorham, Jing Cao},
  journal = {Proc. SPIE Int.Soc.Opt.Eng.},
  volume = {4858},
  pages = {12},
  issue = {31},
  year = {2003},
  month = {March},
  doi = {10.1117/12.458018},
  url = {http://spie.org/Publications/Proceedings/Paper/10.1117/12.458018},
  publisher = {SPIE Proceedings}
}


@article{seckel_2001,
  title = {Neutrinos from propagation of ultrahigh energy protons},
  author = {Engel, Ralph and Seckel, David and Stanev, Todor},
  journal = {Phys. Rev. D},
  volume = {64},
  issue = {9},
  pages = {093010},
  numpages = {10},
  year = {2001},
  month = {Oct},
  doi = {10.1103/PhysRevD.64.093010},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.64.093010},
  publisher = {American Physical Society}
}

@article{Torres_2004,
  title = {Astrophysical origins of ultrahigh energy cosmic rays},
  author = {Torres, Diego F and Anchordoqui, Luis A},
  journal = {Rep. Prog. Phys},
  volume = {67},
  year = {2004},
  pages = {1663-1730}
}

@article{Fermi_1949,
  title = {On the Origin of the Cosmic Radiation},
  author = {Fermi, Enrico},
  journal = {Physical Review},
  volume = {75},
  number = {8},
  year = {1949},
  pages = {1169-1174}
}
















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

@string{aa = "Astron.~Astrophys."}

@string{asr = "Adv.~Space~Res."}

@string{ang = "Ann.~Geophys."}

@string{ao = "Appl.~Opt."}

@string{apj="Apj"}

@string{araa="Ann.~Rev.~Astron.~Astrophys."}

@string{asr="Adv.~Space.~Res."}

@string{baas="Bull.~Am.~Astron.~Soc."}

@string{bams="Bull.~Am.~Meteorol.~Soc."}

@string{blm="Boundary-layer Meteorol."}

@string{bpa2 = "Beitr.~Phys.~Atmosph." }

@string{cap="Contrib.~Atmos.~Phys."}

@string{cc  = "Climatic~Change"}

@string{cup  = "Cambridge~University~Press"}

@string{gfd="Geophys.~Fluid~Dyn."}

@string{grl="Geophys.~Res.~Lett."}

@string{ijep= "Int.~J.~Environment and Pollution"}

@string{iaop= "Izvestiya,~Atmos.~Ocean.~Phys."}

@string{ica= "Icarus"}

@string{jam = "J.~Appl.~Met."}

@string{jas = "J.~Atmos.~Sci."}

@string{jfm = "J.~Fluid~Mech."}

@string{jgr = "J.~Geophys.~Res."}

@string{josa = "J.~Opt.~Soc.~Am."}

@string{jpo = "J.~Phys.~Oceanogr."}

@string{jqsrt = "J.~Spectrosc.~Radiat.~Transfer"}

@string{jqsrt="J.~Quant.~Spectrosc.~Radiat.~Transfer"}

@string{jweia="J.~Wind~Eng.~Indust.~Aerodyn."}

@string{lps="Lunar Planet Sci."}

@string{mwr = "Monthly Weather Rev." }

@string{pss="Plan.~Space~Sci."}

@string{ptrsl="Phil.~Trans.~R.~Soc.~London"}

@string{qjr = "Q.~J.~R.~Meteorol.~Soc."}

@string{qjrms="Q.~J.~R.~Meteorol.~Soc."}

@string{rg="Rev.~Geophys."}

@string{sci="Science"}

@string{sjssc="Siam J.~Sci.~Stat.~Comput."}

@string{ssr = "Space Science Rev." }

@string{tel="Tellus"}

@Book{Example,
  author =	 {Andrews, D. G. and Holton, J. R. and Leovy, C. B.},
  title = 	 {Middle Atmosphere Dynamics},
  publisher = 	 {Academic {P}ress},
  year = 	 1987
}

@BOOK{Bagnold:1954,
   AUTHOR    = {Bagnold, R. A.},
   TITLE     = {The Physics of Blown Sand and Desert Dunes},  
   YEAR      = {1954},
   PUBLISHER = {Methuen},
}

@INCOLLECTION{CLIMSYSMOD:15,
   AUTHOR    = {Brasseur, G. P. and Madronich, S.},
   TITLE     = {Tracer Transport},  
   BOOKTITLE = {Climate System Modeling},  
   PUBLISHER = {Cambridge University Press},
   YEAR      = {1992},
     EDITOR  = {Trenberth, K. E.},
     CHAPTER = {15},
     PAGES   = {491-517}
}

@Book{Chang:1977,
  editor =	 {Chang, J.},
  title = 	 {Methods in computational physics},
  publisher = 	 {Academic {P}ress},
  year = 	 1977,
  volume =	 17
}

@Article{Dunkerton:1981,
  author = 	 {Dunkerton, T. J. and Hsu, C.-P. F. and Mc{I}ntyre, M. E.},
  title = 	 {Some {E}ulerian and {L}agrangian diagnostics for a model stratospheric warming},
  journal = 	 jas,
  year = 	 1981,
  volume =	 38,
  pages =	 {819-843}
}

@Article{Eliassen:1961,
  author = 	 {Eliassen, A. and Palm, E.},
  title = 	 {On the transfer of energy in stationary mountain waves},
  journal = 	 {Geofys. Publ.},
  year = 	 1961,
  volume =	 22,
  number =	 3,
  pages =	 {1-23}
}

@Article{Emanuel:1991,
  author = 	 {Emanuel, K. A.},
  title = 	 {A scheme for representing cumulus convection in large scale models},
  journal = 	JAS,
  year = 	 1991,
  volume =	 48,
  pages =	 {2313-2335}
}

@Book{Emanuel:1994,
  author =	 {Emanuel, K. A.},
  title = 	 {Atmospheric Convection},
  publisher = 	 {Oxford University Press},
  year = 	 1994
}

@Article{Forget:1999,
  author = 	 {Forget, F. and Hourdin, F. and Fournier, F. and Hourdin, C. and Talagrand, O. and Collins, M. and Lewis, S. R. and Read, P. L. and Huot, J.-P.},
  title = 	 {Improved general circulation models of the {M}artian atmosphere from the surface to above 80 km},
  journal = 	 jgr,
  year = 	 1999,
  volume =	 104,
  number =	 {E10},
  pages =	 {24155-24175}
}


@ARTICLE{Hoskins:1975,
   AUTHOR  = {Hoskins, B. J. and Simmons, A. J.},
   TITLE   = {A Multi-Layer Spectral Model and the Semi-Implicit Method},  
   YEAR    = {1975},
   JOURNAL = qjrms,
     VOLUME  = {101},
     PAGES   = {637-655}
}



@unpublished{SURF_design,
	AUTHOR 	= {Allison, P},
	TITLE 	= {SURF Design},
	YEAR 	= {2014},
	NOTE = {ANITA ELOG},
	MONTH 	= {January},
}

\end{references}

